RankAdaptor: Hierarchical Rank Allocation for Efficient Fine-Tuning Pruned LLMs via Performance Model

The efficient compression of large language models (LLMs) has become increasingly popular. However, recovering the performance of compressed LLMs remains a major challenge. The current practice in LLM compression entails the implementation of structural pruning, complemented by a recovery phase that leverages the Low-Rank Adaptation (LoRA) algorithm. Structural pruning's uneven modification of model architecture, coupled with standard LoRA's fixed configuration allocation across layers in an online pipeline, leads to suboptimal performance in various downstream tasks for pruned models. To address this challenge, we introduce RankAdaptor, a hierarchical rank allocation method that enables efficient fine-tuning of pruned LLMs according to layerwise specific recovery requirements. We employ a performance model that conducts offline meta-learning and online incremental learning to explore optimal rank values for each layer. Comprehensive experiments on popular benchmarks show that RankAdaptor consistently outperforms state-of-the-art methods across a variety of pruning settings and LLM architectures, with improvements ranging from 0.7\% to 5.5\%.

==> tabs/mov.tex <==
\begin{table}
    \centering
    \caption{Rank Value Configurations. Fixed refers to applying a constant rank value across multiple layers of the pruned model, while Different indicates assigning distinct rank values to different layers of the pruned model.}
    \begin{tabular}{c|c|c}
        \hline
        \text{Layer}  & \text{Fixed} & \text{Different} \\
        \hline
        1--8  & \multirow{4}{*}{8} & 4 \\
        9--16  &  & 6 \\
        17--24  &  & 10 \\
        25--32  &  & 12 \\
        \hline
    \end{tabular}
    \label{tab: moti_config}
\end{table}

==> tabs/res-llama7b-avg.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the overall performance across multiple tasks. The results are reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc|c}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA & Average \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40 & 63.10 \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 & 56.96 \\
            \cmidrule{2-10}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60 & 59.52  \\
            \cmidrule{2-10}
            & RankAdaptor & 66.91 & 76.93 & 68.78 & 63.14 & 65.24 & 37.54 & 40.80 & \textbf{59.90}  \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 & 54.63 \\
            \cmidrule{2-10}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40 & 57.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 63.15 & 75.95 & 65.97 & 62.04 & 62.63 & 36.77 & 39.60 & \textbf{58.16} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 & 52.58 \\
            \cmidrule{2-10}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60 & 56.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 62.72 & 74.39 & 63.61 & 63.14 & 60.10 & 33.62 & 40.20 & \textbf{56.97} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 57.98 & 60.94 & 34.35 & 52.25 & 31.82 & 27.30 & 35.80 & 42.92 \\
            \cmidrule{2-10}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & 28.75 & 34.60 & 45.62   \\
            \cmidrule{2-10}
            & RankAdaptor & 51.65 & 69.48 & 45.03 & 51.93 & 45.66 & 28.41 & 35.00 & \textbf{46.74}  \\
            \bottomrule
        \end{tabular}
    }\label{tab: res-llama7b-avg}
\end{table*}

==> tabs/tab__ablation.tex <==
\begin{table*}[ht]
\centering
\caption{Ablation study results comparing performance across seven tasks using LLM-Pruner on LLaMA-7B. 'Bold' indicates better performance. The results are reported in percentage (\%).}
\label{tab: Ablation}
\resizebox{\linewidth}{!}
{
\begin{tabular}{c|cc|ccc|cc|ccc}
\toprule
\multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Sample Size} & \multicolumn{3}{c}{Micro-batch Size} & \multicolumn{2}{c}{Element-wise Importance} & \multicolumn{3}{c}{Setting of Performance Model} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-11}
 & $N$=10 & $N$=50 & Micro-4 & Micro-8 & Micro-16 & Element\textsuperscript{1} & Element\textsuperscript{2} & Setting1 & Setting2 & Setting3 \\
\midrule
ARC-e       & 63.97 & \textbf{65.32} & 64.52 & 63.97 & \textbf{65.24} & \textbf{63.97} & 62.84 & 63.97 & 64.73 & 64.65 \\
ARC-c       & 37.29 & \textbf{37.71} & \textbf{38.65} & 37.29 & 37.54 & \textbf{37.29} & 36.77 & 37.29 & 36.60 & \textbf{37.54} \\
WinoG  & \textbf{63.61} & 63.14 & 62.04 & \textbf{63.61} & 63.14 & \textbf{63.61} & 63.22 & 63.61 & \textbf{63.46} & 63.06 \\
OBQA        & \textbf{39.80} & \textbf{41.00} & 40.00 & 39.80 & \textbf{40.80} & \textbf{39.80} & 39.80 & 39.80 & \textbf{40.80} & \textbf{40.80} \\
BoolQ       & \textbf{65.81} & 64.43 & \textbf{67.28} & 65.81 & 66.91 & 65.81 & \textbf{66.48} & \textbf{66.91} & 64.43 & 64.86 \\
PIQA        & 76.99 & \textbf{77.15} & 76.50 & \textbf{76.99} & 76.93 & \textbf{76.99} & 76.82 & 76.99 & 76.99 & \textbf{77.04} \\
HellaS   & \textbf{68.56} & 68.52 & 68.08 & 68.56 & \textbf{68.78} & \textbf{68.56} & 67.88 & 68.56 & 68.75 & \textbf{69.00} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tabs/tab__adalora_vs_lora.tex <==
\begin{table}[tb!]
\centering
\caption{Zero-shot performance comparison between AdaLoRA \cite{zhang2023adaptive} and LoRA \cite{hu2021lora}. 'Bold' indicates better performance. 'Avg Diff' represents the average performance difference between AdaLoRA and LoRA across all benchmarks. The results are reported in percentage (\%).}
\label{tab: adalora_lora}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
Method  & BoolQ          & PIQA           & HellaS         & WinoG          & ARC-e          & ARC-c          & OBQA           & Avg Diff \\
\midrule
AdaLoRA & 61.90          & 76.31          & 67.82          & 62.57          & \textbf{64.02} & 36.70          & 40.40          & \multirow{2}{*}{\textbf{0.56}} \\
LoRA    & \textbf{63.30} & \textbf{76.82} & \textbf{68.68} & \textbf{63.38} & 63.76          & \textbf{37.11} & \textbf{40.60} & \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tabs/tab__con-llama7b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Specific value of the rank configuration explored by RankAdaptor in LLaMA-7B pruned by LLM-Pruner}
    \resizebox{0.9\linewidth}{!}
    {
        \begin{tabular}{cc|c}
            \toprule
             Pruning Rate &Tasks& Layers' Rank Values (1\textasciitilde 32/40) \\
            \midrule
              \multirow{7}{*}{20\%} & BoolQ & 8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 2, 2, 4, 10, 10, 6, 10, 10, 10, 6, 6, 2, 2, 10, 2, 4, 2, 10, 10, 10, 4, 10, 10, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 10, 4, 10, 4, 6, 6, 2, 10, 8, 12, 12, 10, 12, 12, 10, 6, 6, 8, 8, 10, 6, 6, 12, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{25\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 2, 2, 10, 10, 2, 10, 10, 10, 2, 2, 2, 4, 10, 4, 6, 10, 2, 2, 6, 10, 2, 2, 10, 10, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 4, 12, 8, 2, 2, 12, 2, 10, 12, 2, 12, 12, 10, 8, 12, 4, 6, 6, 4, 10, 4, 2, 10, 10, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 1, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 12, 10, 4, 4, 6, 2, 12, 8, 8\\
            \cmidrule{1-3}
              \multirow{7}{*}{30\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 6, 10, 4, 2, 4, 2, 4, 12, 8, 2, 2, 2, 12, 12, 12, 12, 2, 12, 4, 4, 2, 10, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{50\%} & BoolQ & 8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
            \bottomrule
        \end{tabular}
    }\label{tab: con-llama7b}
\end{table*}

==> tabs/tab__main.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of pruned LLaMA-7B with AdaLoRA, LoRA, and RankAdaptor recovery. 'Bold' indicates the best performance at each pruning rate. 'Avg' represents the average performance across all benchmarks. Specific rank configurations explored by RankAdaptor are listed in Appendix \ref{app:r}. Reported in percentage (\%).}
    \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{cc|l|ccccccc|c}
            \toprule
            \multicolumn{2}{c|}{Pruning Stage} & Recover & BoolQ & PIQA & HellaS & WinoG & ARC-e & ARC-c & OBQA & Avg \\
            \midrule
            \multirow{12}{*}{\rotatebox[origin=c]{90}{LLM-Pruner}} 
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} 
            & AdaLoRA & 61.90 & 76.31 & 67.82 & 62.57 & 64.02 & 36.70 & 40.40 & 58.53 \\
            & & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60 & 59.09 \\
            & & RankAdaptor & \textbf{67.34} & \textbf{77.31} & \textbf{69.07} & \textbf{64.17} & \textbf{65.36} & \textbf{37.80} & \textbf{41.60} & \textbf{60.38} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} 
            & AdaLoRA & 60.31 & 75.82 & 64.57 & 61.30 & 61.88 & 35.10 & 39.00 & 56.85 \\
            & & LoRA  & 61.93 & 76.01 & \textbf{66.08} & 61.96 & 62.21 & 35.92 & 39.40 & 57.64 \\
            & & RankAdaptor & \textbf{67.43} & \textbf{76.06} & 65.97 & \textbf{64.40} & \textbf{62.63} & \textbf{36.77} & \textbf{40.40} & \textbf{59.09} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} 
            & AdaLoRA & 59.85 & 73.30 & 61.53 & 60.12 & 59.67 & 33.21 & 38.80 & 55.21 \\
            & & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60 & 56.35 \\
            & & RankAdaptor & \textbf{66.21} & \textbf{75.19} & \textbf{63.61} & \textbf{63.14} & \textbf{60.10} & \textbf{34.64} & \textbf{40.20} & \textbf{57.58} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 38.25 & 67.86 & 42.80 & 48.32 & 42.20 & 26.31 & 32.80 & 42.65 \\
            & & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & \textbf{45.66} & \textbf{28.75} & 34.60 & 45.40 \\
            & & RankAdaptor & \textbf{51.65} & \textbf{69.48} & \textbf{45.03} & \textbf{51.93} & 45.20 & 28.41 & \textbf{35.00} & \textbf{46.67} \\
            \midrule
            \multirow{12}{*}{\rotatebox[origin=c]{90}{Shortened}} 
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} 
            & AdaLoRA & 70.14 & 73.85 & 68.92 & 65.73 & 64.93 & 37.12 & 39.34 & 60.00 \\
            & & LoRA  & 71.82 & \textbf{75.31} & 70.50 & 67.36 & 64.40 & 38.60 & 40.80 & 61.26 \\
            & & RankAdaptor & \textbf{74.53} & 75.22 & \textbf{72.81} & \textbf{69.92} & \textbf{66.72} & \textbf{40.23} & \textbf{42.31} & \textbf{63.11} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} 
            & AdaLoRA & 67.93 & 71.54 & 65.23 & 63.14 & 61.83 & 35.53 & 36.13 & 57.33 \\
            & & LoRA  & 69.67 & 73.20 & 66.85 & 64.50 & 63.32 & 37.02 & 37.40 & 58.85 \\
            & & RankAdaptor & \textbf{72.32} & \textbf{75.13} & \textbf{68.91} & \textbf{66.82} & \textbf{65.24} & \textbf{38.54} & \textbf{38.92} & \textbf{60.84} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} 
            & AdaLoRA & 61.83 & 69.72 & 61.24 & 62.34 & 58.13 & 33.23 & 35.54 & 54.58 \\
            & & LoRA  & 63.58 & 71.21 & 62.75 & 63.80 & \textbf{59.42} & 34.50 & 36.80 & 56.01 \\
            & & RankAdaptor & \textbf{66.23} & \textbf{73.42} & \textbf{64.82} & \textbf{65.93} & 59.31 & \textbf{35.84} & \textbf{38.13} & \textbf{57.67} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 44.93 & 61.24 & 41.83 & 52.84 & 42.93 & 28.73 & 32.24 & 43.53 \\
            & & LoRA  & 46.52 & \textbf{62.76} & 43.12 & 54.37 & 44.10 & \textbf{30.07} & 33.50 & 44.92 \\
            & & RankAdaptor & \textbf{48.94} & 62.43 & \textbf{45.24} & \textbf{56.53} & \textbf{46.14} & 29.82 & \textbf{34.84} & \textbf{46.28} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: res-llama7b}
\end{table*}

==> tabs/tab__mov.tex <==
\begin{table}
    \centering
    \caption{Rank Value Configurations. Fixed refers to applying a constant rank value across multiple layers of the pruned model, while Different indicates assigning distinct rank values to different layers of the pruned model.}
    \begin{tabular}{c|c|c}
        \hline
        \text{Layer}  & \text{Fixed} & \text{Different} \\
        \hline
        1--8  & \multirow{4}{*}{8} & 4 \\
        9--16  &  & 6 \\
        17--24  &  & 10 \\
        25--32  &  & 12 \\
        \hline
    \end{tabular}
    \label{tab: moti_config}
\end{table}

==> tabs/tab__res-llama13b.tex <==
\begin{table*}[tb!]
    \centering
    \caption{Zero-shot performance of pruned LLaMA-13B with AdaLoRA, LoRA, and RankAdaptor recovery. 'Bold' indicates the best performance at each pruning rate. 'Avg' represents the average performance across all benchmarks. The results are reported in percentage (\%).}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{cc|l|ccccccc|c}
            \toprule
            \multicolumn{2}{c|}{Pruning Stage} & Recover & BoolQ & PIQA & HellaS & WinoG & ARC-e & ARC-c & OBQA & Avg \\
            \midrule
            \multirow{3}{*}{\rotatebox[origin=c]{90}{LLM-}\rotatebox[origin=c]{90}{Pruner}}  
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 59.63 & 69.03 & 51.61 & 51.24 & 50.76 & 28.25 & 35.70 & 49.46 \\
            & & LoRA  & 61.93 & 71.38 & \textbf{53.36} & 53.59 & 53.11 & 29.95 & 38.00 & 51.62 \\
            & & RankAdaptor & \textbf{62.05} & \textbf{71.71} & 53.33 & \textbf{54.22} & \textbf{53.20} & \textbf{30.89} & \textbf{39.40} & \textbf{52.11} \\
            \midrule
            \multirow{3}{*}{\rotatebox[origin=c]{90}{Shortened}} 
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 71.53 & 70.92 & 54.32 & 52.83 & 50.94 & 31.62 & 39.21 & 53.05 \\
            & & LoRA  & 73.75 & \textbf{73.81} & 55.96 & 54.41 & 52.35 & 32.81 & 40.60 & 54.81 \\
            & & RankAdaptor & \textbf{75.92} & 72.64 & \textbf{57.83} & \textbf{56.23} & \textbf{54.12} & \textbf{33.96} & \textbf{41.92} & \textbf{56.09} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: res-llama13b}
\end{table*}

==> tabs/tab__res-llama7b-avg.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the overall performance across multiple tasks. The results are reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc|c}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA & Average \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40 & 63.10 \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 & 56.96 \\
            \cmidrule{2-10}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60 & 59.52  \\
            \cmidrule{2-10}
            & RankAdaptor & 66.91 & 76.93 & 68.78 & 63.14 & 65.24 & 37.54 & 40.80 & \textbf{59.90}  \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 & 54.63 \\
            \cmidrule{2-10}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40 & 57.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 63.15 & 75.95 & 65.97 & 62.04 & 62.63 & 36.77 & 39.60 & \textbf{58.16} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 & 52.58 \\
            \cmidrule{2-10}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60 & 56.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 62.72 & 74.39 & 63.61 & 63.14 & 60.10 & 33.62 & 40.20 & \textbf{56.97} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 57.98 & 60.94 & 34.35 & 52.25 & 31.82 & 27.30 & 35.80 & 42.92 \\
            \cmidrule{2-10}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & 28.75 & 34.60 & 45.62   \\
            \cmidrule{2-10}
            & RankAdaptor & 51.65 & 69.48 & 45.03 & 51.93 & 45.66 & 28.41 & 35.00 & \textbf{46.74}  \\
            \bottomrule
        \end{tabular}
    }\label{tab: res-llama7b-avg}
\end{table*}

==> tabs/tab__res-vicuna7b.tex <==
\begin{table*}[tb!]
    \centering
    \caption{Zero-shot performance of pruned Vicuna-7B with AdaLoRA, LoRA, and RankAdaptor recovery. 'Bold' indicates the best performance at each pruning rate. 'Avg' represents the average performance across all benchmarks. The results are reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cc|l|ccccccc|c}
            \toprule
            \multicolumn{2}{c|}{Pruning Stage} & Recover & BoolQ & PIQA & HellaS & WinoG & ARC-e & ARC-c & OBQA & Avg \\
            \midrule
            \multirow{12}{*}{\rotatebox[origin=c]{90}{LLM-Pruner}}  
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} 
            & AdaLoRA & 55.43 & 75.22 & 65.31 & 60.89 & 64.96 & 35.61 & 38.10 & 56.50 \\
            & & LoRA  & 57.77 & \textbf{77.58} & 67.16 & 63.14 & 67.30 & 37.71 & 40.40 & 58.72 \\
            & & RankAdaptor & \textbf{61.19} & 77.15 & \textbf{67.32} & \textbf{63.85} & \textbf{67.68} & \textbf{38.05} & \textbf{41.20} & \textbf{59.49} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} 
            & AdaLoRA & 48.24 & 72.89 & 62.25 & 59.18 & 61.58 & 33.57 & 38.30 & 53.72 \\
            & & LoRA  & 50.34 & 75.24 & 64.10 & 61.33 & \textbf{63.93} & 35.67 & 40.60 & 55.89 \\
            & & RankAdaptor & \textbf{58.50} & \textbf{76.17} & \textbf{64.23} & \textbf{61.96} & 63.30 & \textbf{36.01} & \textbf{42.00} & \textbf{57.45} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} 
            & AdaLoRA & 56.46 & 71.87 & 58.85 & 58.27 & 56.66 & 31.69 & 36.50 & 52.90 \\
            & & LoRA  & \textbf{58.81} & 74.37 & 60.70 & \textbf{60.62} & 59.01 & 33.79 & 38.80 & 55.16 \\
            & & RankAdaptor & 57.58 & \textbf{75.57} & \textbf{61.63} & 60.22 & \textbf{60.94} & \textbf{34.81} & \textbf{39.00} & \textbf{55.68} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 57.21 & 64.52 & 41.83 & 49.66 & 46.05 & 24.35 & 31.70 & 45.05 \\
            & & LoRA  & \textbf{59.51} & 66.87 & 43.18 & \textbf{52.01} & 48.40 & 26.45 & 34.00 & 47.20 \\
            & & RankAdaptor & 59.91 & \textbf{67.46} & \textbf{43.50} & 52.41 & \textbf{48.70} & \textbf{27.65} & \textbf{35.80} & \textbf{47.92} \\
            \midrule
            \multirow{12}{*}{\rotatebox[origin=c]{90}{Shortened}} 
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} 
            & AdaLoRA & 69.52 & 72.95 & 66.83 & 63.91 & 65.82 & 37.23 & 38.64 & 59.27 \\
            & & LoRA  & 71.82 & 74.32 & 68.45 & \textbf{67.62} & 67.35 & 38.50 & 39.80 & 61.12 \\
            & & RankAdaptor & \textbf{74.31} & \textbf{76.92} & \textbf{70.73} & 65.37 & \textbf{69.51} & \textbf{40.12} & \textbf{41.34} & \textbf{62.61} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} 
            & AdaLoRA & 67.63 & 71.84 & 64.15 & 62.53 & 62.41 & 36.72 & 37.32 & 57.51 \\
            & & LoRA  & 69.85 & 73.21 & 65.72 & 64.08 & 63.90 & \textbf{39.32} & 38.50 & 59.23 \\
            & & RankAdaptor & \textbf{72.41} & \textbf{75.62} & \textbf{67.93} & \textbf{66.21} & \textbf{65.84} & 37.95 & \textbf{39.91} & \textbf{60.84} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} 
            & AdaLoRA & 60.92 & 70.54 & 59.21 & 61.15 & 56.73 & 33.42 & 35.61 & 53.94 \\
            & & LoRA  & 62.75 & 71.93 & 60.68 & 62.70 & \textbf{60.32} & 34.50 & 36.80 & 55.67 \\
            & & RankAdaptor & \textbf{65.13} & \textbf{74.21} & \textbf{62.84} & \textbf{64.92} & 58.15 & \textbf{35.93} & \textbf{38.12} & \textbf{57.04} \\
            \cmidrule{2-11}
            & \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} 
            & AdaLoRA & 58.63 & 66.42 & 45.21 & 52.34 & 46.92 & 27.51 & 33.42 & 47.21 \\
            & & LoRA  & 60.37 & \textbf{69.73} & 46.50 & 53.76 & 48.25 & 28.72 & 34.60 & 48.85 \\
            & & RankAdaptor & \textbf{62.54} & 67.88 & \textbf{48.12} & \textbf{55.62} & \textbf{49.84} & \textbf{29.91} & \textbf{35.83} & \textbf{49.96} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: res-vicuna7b}
\end{table*}

==> tabs/tab__wo_ft.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of pruned LLaMA-7B without recovery. 'Avg' represents the average performance across all benchmarks. The results are reported in percentage (\%).}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{cc|ccccccc|c}
            \toprule
            \multicolumn{2}{c|}{Pruning Stage} & BoolQ & PIQA & HellaS & WinoG & ARC-e & ARC-c & OBQA & Avg \\
            \midrule
            \multirow{4}{*}{\rotatebox[origin=c]{90}{LLM-Pruner}}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 20\%}} & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 & 56.68 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 25\%}} & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 & 54.92 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 30\%}} & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 & 52.87 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 50\%}} & 57.98 & 60.94 & 34.35 & 52.25 & 31.82 & 27.30 & 35.80 & 42.92 \\
            \midrule
            \multirow{4}{*}{\rotatebox[origin=c]{90}{Shortened}} 
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 20\%}} & 62.65 & 77.24 & 68.83 & 61.26 & 62.76 & 37.52 & 40.99 & 58.75 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 25\%}} & 61.74 & 74.69 & 64.22 & 60.56 & 57.48 & 35.94 & 40.58 & 56.46 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 30\%}} & 60.73 & 74.64 & 59.84 & 59.64 & 53.75 & 33.31 & 39.55 & 54.49 \\
            \cmidrule{2-10}
            & \multirow{1}{*}{\parbox{1.8cm}{Rate = 50\%}} & 59.72 & 62.16 & 35.38 & 53.81 & 32.77 & 28.12 & 36.87 & 44.12 \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: res-llama7b-wo}
\end{table*}
